Neutron DVCS Measurements with BONuS12 in CLAS12

The three-dimensional picture of quarks and gluons in the nucleon is set to be revealed through deeply virtual Compton scattering (DVCS). With the absence of a free neutron target, the deuterium target represents the simplest nucleus to be used to probe the internal 3D partonic structure of the neutron. We propose here to measure the beam spin asymmetry (BSA) in incoherent neutron DVCS together with the approved E12-06-113 experiment (BONuS12) within the run group F, using the same beam time, simply with addition of beam polarization. The DVCS BSA on the quasi-free neutron will be measured in a wide range of kinematics by tagging the scattered electron and the real photon final state with the spectator proton. We will also measure BSA with all final state particles detected including the struck neutron. The proposed measurements is complementary to the approved CLAS12 experiment E12-11-003, which will also measure the quasi-free neutron DVCS by detecting the scattered neutron, but not the spectator proton. Indeed, besides providing more data for neutron DVCS, this experiment will allow a comparison of the measurement of the BSA of neutron DVCS from the approved E12-11-003 with the measurements using the two methods proposed herein. This comparison will help to understand the impact of nuclear effects, such as the final state interactions (FSI) and Fermi motion on the measurement of the neutron DVCS.

==> preamble.tex <==
%Tagged EMC specific preamble

% See hyperref documentation for information on those parameters
\usepackage{hyperref}
\hypersetup
{
bookmarksopen=true,
%Group Proposal", %subject of the document
%pdftoolbar=false, % toolbar hidden
pdfmenubar=true, %menubar shown
pdfhighlight=/O, %effect of clicking on a link
colorlinks=true, %couleurs sur les liens hypertextes
pdfpagemode=UseNone, %aucun mode de page
pdfpagelayout=SinglePage, %ouverture en simple page
pdffitwindow=true, %pages ouvertes entierement dans toute la fenetre
linkcolor=linkcol, %couleur des liens hypertextes internes
citecolor=citecol, %couleur des liens pour les citations
urlcolor=linkcol %couleur des liens pour les url
}


